Impact of Redundancy on Resilience in Distributed Optimization and Learning

This report considers the problem of resilient distributed optimization and stochastic learning in a server-based architecture. The system comprises a server and multiple agents, where each agent has its own local cost function. The agents collaborate with the server to find a minimum of the aggregate of the local cost functions. In the context of stochastic learning, the local cost of an agent is the loss function computed over the data at that agent. In this report, we consider this problem in a system wherein some of the agents may be Byzantine faulty and some of the agents may be slow (also called stragglers). In this setting, we investigate the conditions under which it is possible to obtain an "approximate" solution to the above problem. In particular, we introduce the notion of $(f, r; \epsilon)$-resilience to characterize how well the true solution is approximated in the presence of up to $f$ Byzantine faulty agents, and up to $r$ slow agents (or stragglers) -- smaller $\epsilon$ represents a better approximation. We also introduce a measure named $(f, r; \epsilon)$-redundancy to characterize the redundancy in the cost functions of the agents. Greater redundancy allows for a better approximation when solving the problem of aggregate cost minimization. In this report, we constructively show (both theoretically and empirically) that $(f, r; \mathcal{O}(\epsilon))$-resilience can indeed be achieved in practice, given that the local cost functions are sufficiently redundant.

==> exp-numerical.old.tex <==
We present a group of simulation results applying our algorithm framework to the problems of \textit{distributed linear regression}. Specifically, we study behavior of Algorithm~\ref{alg} according to our theoretical results in Section~\ref{sec:full-grad}, including the special cases.

\subsubsection{Problem Description}

Consider a synchronous server-based system, where in $n=10$ and $d=2$. Each agent $i\in\{1,...,n\}$ has a data point represented by a triplet $(A_i,B_i,N_i)$ where $A_i$ is a $d$-dimensional row vector, $B_i\in\R$ is a response, and $N_i\in\R$ is a noise value. Specifically, for all $i\in\{1,...,n\}$, 
\begin{equation}
    B_i=A_ix^*+N_i ~ \text{ where } ~x^*=\begin{pmatrix}1\\1\end{pmatrix}.
\end{equation}
The collective data is represented by a triplet of matrices $(A, \, B, \, N)$ where the $i$-th row of $A$, $B$, and $N$ are equal to $A_i$, $B_i$ and $N_i$, respectively. The specific values are as follows.
\begin{equation}
    A=\begin{pmatrix}
        1 & 0 \\
        0.8 & 0.5 \\
        0.5 & 0.8 \\
        0 & 1 \\
        -0.5 & 0.8 \\
        -0.8 & 0.5 \\
        0.3 & -0.7 \\
        0.7 & 0.3 \\
        0.3 & 0.7 \\
        0.7 & -0.3
    \end{pmatrix}, ~ 
    B=\begin{pmatrix}
        %0.91078179 \\  1.33487616 \\ 1.33758823 \\ 1.00334385 \\ 0.21424485 \\ -0.36153888
        0.9108 \\  1.3349 \\ 1.3376 \\ 1.0033 \\ 0.2142 \\ -0.3615 \\ -0.3974 \\ 0.9967 \\ 1.0052 \\ 0.3947
    \end{pmatrix}, ~ \text{ and }
    N=\begin{pmatrix}
        %-0.08921821 \\0.03487616\\0.03758823\\0.00334385\\-0.08575515\\-0.06153888
        -0.0892 \\0.0349 \\0.0376\\0.0033\\-0.0858\\-0.0615\\0.0026\\-0.0033\\0.0052\\-0.0053
    \end{pmatrix}.
\end{equation}
It should be noted that
\begin{align}
    B = A x^{*} + N. \label{eqn:set_equations}
\end{align}
We let $A_S$, $B_S$ and $N_S$ represent matrices of dimensions $\mnorm{S} \times 2$, $\mnorm{S} \times 1$ and $\mnorm{S} \times 1$ obtained by stacking the rows $\{A_i, \, i \in S \}$, $\{B_i, \, i \in S \}$ and $\{N_i, \, i \in S\}$, respectively, in the increasing order of $i$. From~\eqref{eqn:set_equations}, observe that for every non-empty set $S$,
\begin{align}
    B_S = A_S x^{*} + N_S. \label{eqn:set_equations-2}
\end{align}
Recall from basic linear algebra that if $A_S$ is full-column rank, i.e., $\rank{A_S} = d = 2$ then $x^*$ is the unique solution of the set of equations in~\eqref{eqn:set_equations-2}. 
% Note that for every set $S$ with $\mnorm{S} \geq n-2f = 6 - 2 = 4$, the matrix $A_S$ is full rank. Specifically,
Note that in this example, for every set $S$ with $\mnorm{S} \geq 2$, the matrix $A_S$ is full rank. Specifically,
\begin{align}
    \rank{A_S} = d = 2, \quad \forall S \subseteq \{1, \ldots, \, 10\}, ~ \mnorm{S} \geq 2. \label{eqn:exp_full_rank}
\end{align}

In this particular distributed optimization problem, each agent $i$ has a quadratic cost function defined to be 
\[Q_i(x)=(B_i-A_ix)^2, \quad \forall x \in \R^2.\] 
For an arbitrary non-empty set of agents $S$, we define 
\begin{align}
Q_S(x) = \sum_{i\in S}Q_i(x) = \sum_{i \in S}\left(B_i-A_ix \right)^2 = \norm{B_S-A_Sx}^2, \quad \forall x \in \R^2. \label{def:exp_Q_S}
\end{align}
As matrix $A_S$ is full rank for every $S$ with $\mnorm{S} \geq 2$,
\begin{align}
    \arg \min_{x \in \R^2} Q_S(x) = \arg \min_{x \in \R^2} \norm{B_S-A_Sx}^2 = \left(x ~ \vline ~ A_S x = B_S \right). \label{eqn:solve_Q_S}
\end{align}
Therefore, $Q_S(x)$ has a unique minimum point when $\mnorm{S} \geq 2$. Henceforth, we write notation $\arg \min_{x \in \R^2}$ simply as $\arg \min$, unless otherwise stated.

\subsubsection{Redundancy property and parameters}

In the following experiments, we choose $f=0,1,2$ and $r=0,1,2$, with various combinations. In each execution, we always designate the first $f$ agents to be Byzantine faulty. It can be verified first that the agents' cost functions satisfy $(f,r;\epsilon)$-redundancy property. The value of $\epsilon$ can be computed by the following steps, similar to the steps in the previous section:
\begin{enumerate}
    \item For each set $S\subset\{1,...,n\}$ with $\mnorm{S}=n-f$, compute $x_S\in\R^2$ such that $B_S=A_Sx_S$. Note that due to \eqref{eqn:solve_Q_S}, $x_S=\arg\min Q_S(x)$.
    \item For each set $S\subset\{1,...,n\}$ with $\mnorm{S}=n-f$, do the following:
    \begin{enumerate}
        \item For each set $\widehat{S}\subseteq{S}$ with $\mnorm{\widehat{S}}\geq n-2f-r$, compute $x_{\widehat{S}}$ such that $B_{\widehat{S}}=A_{\widehat{S}}x_{\widehat{S}}$. By \eqref{eqn:solve_Q_S}, $x_{\widehat{S}}=\arg\min Q_{\widehat{S}}(x)$.
        \item Compute $\epsilon_S=\max_{\widehat{S}\subseteq S,\mnorm{\widehat{S}}\geq n-2f-r}\norm{x_S-x_{\widehat{S}}}$.
    \end{enumerate}
    \item Finally, compute $\epsilon=\max_{S,\mnorm{S}=n-f}\epsilon_S$.
\end{enumerate}
The values of $\epsilon$ with different $f$ and $r$ are presented in Figure~\ref{fig:trade-off}. We can see that larger the values of $f$ and $r$, larger the value of $\epsilon$, indicating less accurate the algorithm can we expect. 

We simulate the distributed gradient-descent-based algorithm according to Theorem~\ref{thm:async-fault-toler} in Section~\ref{sec:full-grad}. The algorithm ignores the input from $r$ slowest agents in each iteration, and uses the CGE GAR to tolerate Byzantine agents. Let $\H=[n]\backslash[f]$ be the set of non-faulty agents. From \eqref{eqn:solve_Q_S} we can compute the minimum point of the aggregate cost function of non-faulty agents $x_\H=x_S=\sum_{i\in\H}Q_i(x)$.

For each agent $i$, its cost function $Q_i(x)$ has Lipschitz continuous gradients, i.e., satisfies Assumption~\ref{assum:lipschitz}, with Lipschitz coefficient $\mu=2\overline{v}_i$, where $\overline{v}_i$ denotes the largest eigenvalue of $A_i^TA_i$. Also, for the set $S$, their average cost function $(1/\mnorm{S})Q_S(x)$ is strongly convex, i.e., satisfies Assumption~\ref{assum:strongly-convex-ft}, with strong convexity coefficient $\gamma=2\underline{v}_S/\mnorm{S}$, where $\underline{v}_S$ is the smallest eigenvalue of $A_S^TA_S$. The derivations of computing these two coefficients can be found in \cite[Section 10]{gupta2019byzantine}. We can compute the values of the coefficients accordingly: $\mu=2$; $\gamma =0.788, 0.588, 0.439$ when $f=0,1,2$, respectively.

We use the following parameters implementing the algorithm. In update rule \eqref{eqn:update}, we use step size $\eta_t=1.5/(t+1)$ for iteration $t=0,1,...$, which satisfies the conditions $\sum_{t=0}^\infty\eta_t=\infty$ and $\sum_{t=0}^\infty\eta_t^2=3\pi^2/8<\infty$  (see~\cite{rudin1964principles}). We assume the convex compact $\W\subset\R^d$ to be a 2-dimensional hypercube $[-1000,1000]^2$. Note that $x_\H\in\W$. In all simulations presented, the initial estimate $x^0=(0,0)^T$. In every execution, we observe that the iterative estimates produced by the algorithm practically converge after 400 iterations. Thus, to measure the approximate result outputted by the algorithm, we use $x_\textrm{out}=x^{500}$. 

Two types of fault behaviors are simulated: (i) \textit{gradient-reverse}: the faulty agent \textit{reverses} its true gradient. Suppose the correct gradient of a faulty agent $i$ at iteration $t$ is $s_i^t$, the agent $i$ will send the incorrect gradient $g_i^t=-s_i^t$ to the server.
(ii) \textit{random}: the faulty agent sends a randomly chosen vector in $\mathbb{R}^d$. In our experiments, the faulty agent in each iteration chooses i.i.d. Gaussian random vector with mean 0 and a isotropic covariance matrix with standard deviation of 200.

\subsubsection{Experiment results and discussions}

The outputs for with different values of $f$ and $r$ are presented in Table~\ref{tab:results} alongside with plain gradient descent output ($f=r=0$) for comparison. Note that $\dist{x_\H}{x_\textrm{out}}=\norm{x_\H-x_\textrm{out}}$. In all executions, $\dist{x_\H}{x_\textrm{out}}<\D^*$ as indicated by Theorem~\ref{thm:async-fault-toler}. The values of $\D^*$ are presented in Table~\ref{tab:D-star}.

We also plot the processes of Algorithm~\ref{alg} solving the numerical examples of some of these experiments, namely the cases when $f=1$ and $2$, in Figure~\ref{fig:a}, with details of the first 150 iterations of each executions. The process when $f=r=0$, i.e., the synchronous fault-free case is also presented for comparison purpose. Theses plots show that in order to be resilient against Byzantine agents and stragglers, the convergence speed is slightly slowed down and there exists a gap between the algorithm's output and the true solution.

\begin{table*}[t]
    \centering
    \caption{Outputs of Algorithm~\ref{alg} when solving distributed linear regression problems while tolerating different number of stragglers ($r$) and Byzantine faulty agents ($f$). GAR in use: summing $n-r$ gradients when $f=0$, and CGE gradient filter when $f=1,2$. Byzantine faulty agents exhibits two different types of Byzantine faults: \emph{gradient-reverse} and \emph{random}. The resilience of the algorithm is shown by the distance between the outputs and the actual solution to the problem. The true solution to optimization problems $x_\H$ are also listed. %Recall that $x_{\mathrm{out}} = x^{500}$ and $\dist{x_\H}{x_{\mathrm{out}}}=\norm{x_\H-x_{\mathrm{out}}}$.
    }
    \small
    \begin{tabular}[t]{c|c|ccc|c}
        & & $r=0$ & $r=1$ & $r=2$ & $x_\H$ \\
        \hline
        \multirow{2}{*}{$f=0$}& $x_\textrm{out}$ & $\begin{pmatrix}1.0117\\0.9883\end{pmatrix}$ & $\begin{pmatrix}1.0152\\0.9891\end{pmatrix}$ & $\begin{pmatrix}1.0311\\0.9872\end{pmatrix}$ & \multirow{2}{*}{$\begin{pmatrix}1.0117\\0.9883\end{pmatrix}$} \\
        & $\dist{x_\H}{x_\textrm{out}}$ & $\sim0$ & $3.66\times10^{-3}$ & $1.95\times10^{-2}$ \\
        \hline
        $f=1$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0460\\0.9883\end{pmatrix}$ & $\begin{pmatrix}1.0363\\0.9994\end{pmatrix}$ & $\begin{pmatrix}1.0346\\0.9934\end{pmatrix}$ & \multirow{4}{*}{$\begin{pmatrix}1.0460\\0.9883\end{pmatrix}$} \\
        \textit{grad-rev} & $\dist{x_\H}{x_\textrm{out}}$ & $1.48\times10^{-5}$ & $1.47\times10^{-2}$ & $1.24\times10^{-2}$ \\
        \cline{1-5}
        $f=1$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0459\\0.9883\end{pmatrix}$ & $\begin{pmatrix}1.0466\\0.9846\end{pmatrix}$ & $\begin{pmatrix}1.0403\\0.9923\end{pmatrix}$ \\
        \textit{random} & $\dist{x_\H}{x_\textrm{out}}$ & $5.42\times10^{-5}$ & $3.71\times10^{-3}$ & $6.93\times10^{-3}$ \\
        \hline
        $f=2$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0067\\0.9621\end{pmatrix}$ & $\begin{pmatrix}1.0138\\0.9789\end{pmatrix}$ & $\begin{pmatrix}0.9891\\1.0090\end{pmatrix}$ & \multirow{4}{*}{$\begin{pmatrix}1.0445\\0.9876\end{pmatrix}$} \\
        \textit{grad-rev} & $\dist{x_\H}{x_\textrm{out}}$ & $4.56\times10^{-2}$ & $3.19\times10^{-2}$ & $5.94\times10^{-2}$ \\
        \cline{1-5}
        $f=2$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0444\\0.9876\end{pmatrix}$ & $\begin{pmatrix}1.0376\\0.9961\end{pmatrix}$ & $\begin{pmatrix}1.0296\\1.0030\end{pmatrix}$ \\
        \textit{random} & $\dist{x_\H}{x_\textrm{out}}$ & $6.00\times10^{-5}$ & $1.10\times10^{-2}$ & $2.14\times10^{-2}$ \\
    \end{tabular}
    \label{tab:results}
\end{table*}

\begin{table}[t]
    \centering
    \caption{Values of $\D^*$ according to Theorem~\ref{thm:async-fault-toler} and \eqref{eqn:thm2-params}.}
    \small
    \begin{tabular}{c|ccc}
         & $r=0$ & $r=1$ & $r=2$ \\
        \hline
        $f=0$ & 0 & 0.207 & 0.385 \\
        $f=1$ & 0.369 & 0.670 & 0.957 \\
        $f=2$ & 1.251 & 1.748 & 2.467 \\
    \end{tabular}
    \label{tab:D-star}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{img/async-comparison-c.pdf}
    \caption{The process of solving the numerical example using Algorithm~\ref{alg}, illustrated by the changes in losses, i.e. $\sum_{i\in\H}Q_i(x^t)$, and distances, i.e., $\mnorm{x^t-x_\H}$, versus the number of iterations in the algorithm. Columns (a) and (c) are the full processes, while (b) and (d) are details from the initial iterations. The results for fault-free synchronous gradient descent ($f=r=0$) is also presented for comparison.}
    \label{fig:a}
\end{figure*}


==> exp-numerical.tex <==
\label{sub:numerical}

We present a group of simulation results applying our algorithm framework to the problems of \textit{distributed linear regression}. Specifically, we study behavior of Algorithm~\ref{alg} according to our theoretical results in Section~\ref{sec:full-grad}, including the special cases. %A detailed description of these experiments can be found in Appendix~\ref{appdx:exp-numerical}.

Consider a synchronous server-based system, where $n=10$ and $d=2$. Each agent $i\in\{1,...,n\}$ has a data point represented by a triplet $(A_i,B_i,N_i)$ where $A_i$ is a $2$-dimensional row vector, $B_i\in\R$ is a response, and $N_i\in\R$ is a noise value. Specifically, for all $i\in\{1,...,n\}$, {$n=10$,} $B_i=A_ix^*+N_i ~ \text{ where } ~x^*=\begin{pmatrix}1, 1\end{pmatrix}^T$.
The collective data is represented by a triplet of matrices $(A, \, B, \, N)$ where the $i$-th row of $A$, $B$, and $N$ are equal to $A_i$, $B_i$ and $N_i$, respectively. Each agent $i$ has a quadratic cost function defined to be $Q_i(x) = (B_i - A_ix)^2, \forall x\in\R^2$.

% We let $A_S$, $B_S$ and $N_S$ represent matrices of dimensions $\mnorm{S} \times 2$, $\mnorm{S} \times 1$ and $\mnorm{S} \times 1$ obtained by stacking the rows $\{A_i, \, i \in S \}$, $\{B_i, \, i \in S \}$ and $\{N_i, \, i \in S\}$, respectively, in the increasing order of $i$.

In this group of experiments, we choose $f=0,1,2$ and $r=0,1,2$, with various combinations. In each execution, we always designate the first $f$ agents to be Byzantine faulty (labeled 1 through $f$). Stragglers are actual stragglers in each iteration whose gradients are the last $r$ ones received by the server. It can be verified first that the agents' cost functions satisfy $(f,r;\epsilon)$-redundancy property. The values of $\epsilon$ with different $f$ and $r$ are presented in Figure~\ref{fig:trade-off}. We can see that larger the values of $f$ and $r$, larger the value of $\epsilon$, and less accurate the algorithm can we expect. We can also compute the values of the coefficients accordingly: $\mu=2$; $\gamma =0.788, 0.588, 0.439$ when $f=0,1,2$, respectively.

We use the following parameters implementing the algorithm. In update rule \eqref{eqn:update}, we use step size $\eta_t=1.5/(t+1)$ for iteration $t=0,1,...$, which satisfies $\sum_{t=0}^\infty\eta_t=\infty$ and $\sum_{t=0}^\infty\eta_t^2<\infty$. %(see~\cite{rudin1964principles}). 
We assume the convex compact $\W\subset\R^d$ to be a 2-dimensional hypercube $[-1000,1000]^2$. Note that $x_\H\in\W$. In all simulations presented, the initial estimate $x^0=(0,0)^T$. In every execution, we observe that the iterative estimates produced by the algorithm practically converge after 400 iterations. Thus, to measure the approximate result outputted by the algorithm, we use $x_\textrm{out}=x^{500}$. 

Two types of faulty behaviors are simulated: (i) \textit{gradient-reverse}: each faulty agent \textit{reverses} its true gradient. Suppose the correct gradient of a faulty agent $i$ at iteration $t$ is $s_i^t$, the agent $i$ sends the incorrect gradient $g_i^t=-s_i^t$ to the server.
(ii) \textit{random}: the faulty agent sends a randomly chosen vector in $\mathbb{R}^d$. In our experiments, the faulty agent in each iteration chooses i.i.d. Gaussian random vector with mean 0 and a isotropic covariance matrix with standard deviation of 200.

The outputs for with different values of $f$ and $r$ are presented in Table~\ref{tab:results} alongside with plain gradient descent output ($f=r=0$) for comparison. Note that $\dist{x_\H}{x_\textrm{out}}=\norm{x_\H-x_\textrm{out}}$. In all executions, $\dist{x_\H}{x_\textrm{out}}<\D^*$ as indicated by Theorem~\ref{thm:async-fault-toler}. The values of $\D^*$ are listed below.%presented in Table~\ref{tab:D-star}.
\begin{center}
    \footnotesize
    \begin{tabular}{c|ccc}
         & $r=0$ & $r=1$ & $r=2$ \\
        \hline
        $f=0$ & 0 & 0.207 & 0.385 \\
        $f=1$ & 0.369 & 0.670 & 0.957 \\
        $f=2$ & 1.251 & 1.748 & 2.467 \\
    \end{tabular}
\end{center}

We also plot the processes of Algorithm~\ref{alg} solving the numerical examples of some of these experiments, namely the cases when $f=1$ and $2$, in Figure~\ref{fig:a}, with details of the first 150 iterations of each executions. The process when $f=r=0$, i.e., the synchronous fault-free case is also presented for comparison purpose. Theses plots show that in order to be resilient against Byzantine agents and stragglers, the convergence speed is slightly slowed down and there exists a gap between the algorithm's output and the true solution.

\begin{table}[t]
    \centering
    \tiny
    \begin{tabular}[t]{c|c|ccc|c}
        & & $r=0$ & $r=1$ & $r=2$ & $x_\H$ \\
        \hline
        \multirow{2}{*}{$f=0$}& $x_\textrm{out}$ & $\begin{pmatrix}1.0117, 0.9883\end{pmatrix}^T$ & $\begin{pmatrix}1.0152, 0.9891\end{pmatrix}^T$ & $\begin{pmatrix}1.0311, 0.9872\end{pmatrix}^T$ & \multirow{2}{*}{$\begin{pmatrix}1.0117, 0.9883\end{pmatrix}^T$} \\
        & $\dist{x_\H}{x_\textrm{out}}$ & $\sim0$ & $3.66\times10^{-3}$ & $1.95\times10^{-2}$ \\
        \hline
        $f=1$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0460, 0.9883\end{pmatrix}^T$ & $\begin{pmatrix}1.0363, 0.9994\end{pmatrix}^T$ & $\begin{pmatrix}1.0346, 0.9934\end{pmatrix}^T$ & \multirow{4}{*}{$\begin{pmatrix}1.0460, 0.9883\end{pmatrix}^T$} \\
        \textit{grad-rev} & $\dist{x_\H}{x_\textrm{out}}$ & $1.48\times10^{-5}$ & $1.47\times10^{-2}$ & $1.24\times10^{-2}$ \\
        \cline{1-5}
        $f=1$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0459, 0.9883\end{pmatrix}^T$ & $\begin{pmatrix}1.0466, 0.9846\end{pmatrix}^T$ & $\begin{pmatrix}1.0403, 0.9923\end{pmatrix}^T$ \\
        \textit{random} & $\dist{x_\H}{x_\textrm{out}}$ & $5.42\times10^{-5}$ & $3.71\times10^{-3}$ & $6.93\times10^{-3}$ \\
        \hline
        $f=2$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0067, 0.9621\end{pmatrix}^T$ & $\begin{pmatrix}1.0138, 0.9789\end{pmatrix}^T$ & $\begin{pmatrix}0.9891, 1.0090\end{pmatrix}^T$ & \multirow{4}{*}{$\begin{pmatrix}1.0445, 0.9876\end{pmatrix}^T$} \\
        \textit{grad-rev} & $\dist{x_\H}{x_\textrm{out}}$ & $4.56\times10^{-2}$ & $3.19\times10^{-2}$ & $5.94\times10^{-2}$ \\
        \cline{1-5}
        $f=2$ & $x_\textrm{out}$ & $\begin{pmatrix}1.0444, 0.9876\end{pmatrix}^T$ & $\begin{pmatrix}1.0376, 0.9961\end{pmatrix}^T$ & $\begin{pmatrix}1.0296, 1.0030\end{pmatrix}^T$ \\
        \textit{random} & $\dist{x_\H}{x_\textrm{out}}$ & $6.00\times10^{-5}$ & $1.10\times10^{-2}$ & $2.14\times10^{-2}$ \\
    \end{tabular}
    \caption{Outputs of Algorithm~\ref{alg} when solving distributed linear regression in Section~\ref{sub:numerical}. GAR in use: summing $n-r$ gradients when $f=0$, and CGE gradient filter when $f=1,2$. %The resilience of the algorithm is shown by the distance between the outputs and the actual solution to the problem. The true solution to optimization problems $x_\H$ are also listed. %Recall that $x_{\mathrm{out}} = x^{500}$ and $\dist{x_\H}{x_{\mathrm{out}}}=\norm{x_\H-x_{\mathrm{out}}}$.
    }
    \label{tab:results}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{Values of $\D^*$ according to Theorem~\ref{thm:async-fault-toler} and \eqref{eqn:thm2-params}.}
%     \label{tab:D-star}
%     \footnotesize
%     \begin{tabular}{c|ccc}
%          & $r=0$ & $r=1$ & $r=2$ \\
%         \hline
%         $f=0$ & 0 & 0.207 & 0.385 \\
%         $f=1$ & 0.369 & 0.670 & 0.957 \\
%         $f=2$ & 1.251 & 1.748 & 2.467 \\
%     \end{tabular}
% \end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{img/async-comparison-c.pdf}
    \caption{Changes in aggregate cost $\sum_{i\in\H}Q_i(x^t)$, and $\dist{x^t}{x_\H}$, versus the number of iterations with Algorithm~\ref{alg} solving the numerical example. %Columns (a) and (c) are {for the first 500 iterations}, while (b) and (d) are details from the initial iterations. The results for fault-free synchronous gradient descent ($f=r=0$) is also presented for comparison.
    }
    \label{fig:a}
\end{figure*}


==> necessity.tex <==
\section{Necessary condition for $(f,r;\epsilon)$-resilience}
\label{sec:necessity}

We first discuss the necessary condition for achieving $(f,r;\epsilon)$-resilience when solving the RDO problem. Throughout this paper, we make the following assumption.

\begin{assumption}
\label{asp:exists}
For every non-empty set of non-faulty agents $S$, we assume that the set $\arg \min_{x \in \W} \sum_{i \in S}Q_i(x)$ is non-empty and closed. 
\end{assumption}

We also assume that $f < n/2$. Lemma~\ref{lem:n_2f} below shows that $(f, r; \epsilon)$-resilience is impossible in general when $f \geq n/2$. 

\begin{lemma}[\citep{liu2021approximate-full}]
\label{lem:n_2f}
If $f \geq n/2$ then there cannot exist a deterministic $(f, r; \epsilon)$-resilient algorithm for any $\epsilon \geq 0$.
\end{lemma}

Note that $n>f+r$ is also needed to keep the problem valid. We now state our necessity result.

\begin{theorem}
\label{thm:necc}
Suppose that Assumption~\ref{asp:exists} holds true. There exists a deterministic $(f,r;\epsilon)$-resilient distributed optimization algorithm where $\epsilon \geq 0$ {\em only if} the agents' cost functions satisfy the $(f,r;\epsilon)$-redundancy property, if the possible honest cost functions are unknown to the server.
\end{theorem}

\begin{proof} 
We assume that stragglers are extreme enough that none of their information can be received by the server. If a condition is necessary in this particular scenario then it is also necessary in the general case we consider.

% To prove the necessary condition, we also assume that the server has full knowledge of all the agents' cost functions. This may not hold true in practice, where instead the server may only have partial information about the agents' cost functions. Indeed, this assumption forces the Byzantine faulty agents to a priori fix their cost functions. However, in reality the Byzantine agents may send arbitrary information over time to the server that need not be consistent with a fixed cost function. Thus, necessity of $(2f,\epsilon)$-redundancy under this strong assumption implies its necessity in general. 

The proof is by contradiction. Specifically, we show that \textit{if the cost functions of non-faulty agents do not satisfy the $(f,r;\epsilon)$-redundancy property then there cannot exist a \emph{deterministic} $(f,r;\epsilon)$-resilient distributed optimization algorithm.}

For each non-empty subset of agents $T$, we define
\[X_T = \arg \min_x \sum_{i \in T} Q_i(x).\]
In the remainder of this proof, we consider this problem if $f$ and $r$ cannot be 0 at the same time, since if $f=r=0$ the problem is trivial.

Suppose that the agents' cost functions \textbf{do not} satisfy the $(f,r;\epsilon)$-redundancy property stated in Definition~\ref{def:redundancy}. Then, there exists a real number $\delta>0$ and a pair of non-empty subsets of non-faulty agent $S,\widehat{S}$ with $\widehat{S} \subset S$, $\mnorm{S} = n-f$, and $n-2f-r \leq \mnorm{\widehat{S}} < n-f$ such that
\begin{align}
    \dist{X_{\widehat{S}}}{X_S} = \epsilon + \delta. \label{eqn:no_red_asp}
\end{align}

Now, suppose that the subset of the remainder set $\B\subseteq\{1,...,n\}\backslash S$ contains all Byzantine faulty agents. Note that $\B$ is non-empty with $\mnorm{\B}\leq n-\mnorm{S}=f$. 
% Similar to the non-faulty agents, the faulty agents send to the server cost functions that are scalar, and the aggregate of one or more agents' cost functions in the set $S \cup \B$ is unique\footnote{For otherwise Byzantine agents would have been spotted by the server and become useless.}. 
Let us denote the set of non-faulty agents $T=S\backslash\widehat{S}$, with $1\leq\mnorm{T}\leq f+r$. For each agent in $T$, we replace it with one different agent from $\B$ (i.e., a one-to-one mapping from $T$ to $\B$), and denote the new set of agents as $T'$.

The cost functions of faulty agents can be arbitrary. We would like to choose those functions of the faulty agents such that
% \begin{quote}
the aggregate cost function of the agents in the set $\widehat{S}\cup T'$, or $X_{\widehat{S}\cup T'}\triangleq\arg\min_{x}\sum_{i\in\widehat{S}\bigcup T'}Q_i(x)$, to be $\dist{X_{\widehat{S}}}{X_{S}}$ distance away from $X_{\widehat{S}}$, the same as $X_S$, but lies on the opposite side of $X_{\widehat{S}}$ with respect to $X_S$ (i.e., a position that maximizes $\dist{X_S}{X_{\widehat{X}\bigcup T'}}$), as shown in the figure below. Note that it is always possible to pick such functions for the faulty agents. 
\begin{center}
    \includegraphics[width=.8\textwidth]{tikz3.pdf}
\end{center}
Note that the distance between the two sets $X_S$ and $X_{\widehat{S}\cup T'}$ 
\begin{align}
    \dist{x_S}{x_{\widehat{S}\cup T'}} \geq 2(\epsilon + \delta). \label{eqn:dist_x1_x2}
\end{align}

% For example, suppose $S=\{1,2,3,4\}$, $\widehat{S}=\{1,2\}$, $f=r=1$. $Q_1(x)=Q_2(x)=Q_3(x)=x^2$, and $Q_4(x)=(x-1)^2$. $\B$ should contain 1 agent, and we let it be agent 5. $T=\{3,4\}$. If $T'=\{3,5\}$, we can choose $Q_5(x)=(x+1)^2$. If $T'=\{4,5\}$, we can choose $Q_5(x)=x^2+4x$. Either way, $x_{\widehat{S}}=0$, $x_S=1/4$, and $x_{\widehat{S}\cup T'}=-1/4$.

% The functions can be constructed. Suppose each cost function $Q_i(x)$, $i\in S_0$ satisfies $Q_i(x)=Q_i(2x_0-x)$. To satisfy the conditions stated above, for every cost function $Q_i(x)$, $i\in S_1$, one can construct another function $Q_j(x)=Q_i(2x_0-x)$, to be the cost function of an agent $j\in S_2$. \\%(See Figure~\ref{fig:constructQ})\\
%$\distance(x_0,x_1)=\distance(x_0,x_2)=\epsilon$. And functions in $S_0$, $S_1$, and $S_2$ are symmetric with respect to $x_0$, meaning for any $Q_i$ in $X_0$, $Q_i(x)=Q_i(2x_0-x)$, and for any $Q_i\in S_1$ and $Q_j\in S_2$, $Q_i(x)=Q_j(2x_0-x),~\forall x$. \\
% We now show below, by contradiction, that there cannot exist a deterministic $(f, \, \epsilon)$-resilient algorithm.\\

Similarly, 

Now, suppose, toward a contradiction, that there exists an $(f, r; \epsilon)$-resilient deterministic optimization algorithm named $\Pi$. As the identity of Byzantine faulty agents is a priori unknown to the server, and the cost functions sent by the Byzantine faulty agents have similar properties as the non-faulty agents, 
% and the faulty cost functions are assumed differentiable and convex, 
the server cannot distinguish between the following two possible scenarios; i) $S$ is the set of non-faulty agents, and ii) $\widehat{S}\cup T'$ is the set of non-faulty agents. Note that both the sets $S$ and $\widehat{S}\cup T'$ contain $n-f$ agents. 
% Thus, the output of algorithm $\Pi$ assumed to be $(f, \, \epsilon)$-resilient should be located within $\epsilon$ distance from the minimum point of the aggregate cost functions of the non-faulty agents in both the scenarios. \\

As the cost functions received by the server are identical in both of the above scenarios, being a deterministic algorithm, $\Pi$ should have identical output in both the cases. We let $\widehat{x}$ denote the output of $\Pi$. In scenario (i) when the set of honest agents is given by $S$ with $\mnorm{S} = n-f$, as $\Pi$ is assumed $(f,r;\epsilon)$-resilient, by Definition~\ref{def:resilience} the output
\begin{align}
    \dist{\widehat{x}}{X_S}\leq\epsilon \label{eqn:scn_1}
\end{align}
as shown in the figure above. Similarly, in scenario (ii) when the set of honest agents is $\widehat{S}\cup T'$ with $\mnorm{\widehat{S}\cup T'} = n-f$,
\begin{align}
    \dist{\widehat{x}}{x_{\widehat{S}\cup T'}} \leq \epsilon. \label{eqn:scn_2}
\end{align}
However,~\eqref{eqn:dist_x1_x2} implies that~\eqref{eqn:scn_1} and~\eqref{eqn:scn_2} cannot be satisfied simultaneously. That is, if $\Pi$ is $(f,r;\epsilon)$-resilient in scenario (i) then it cannot be so in scenario (ii), and vice-versa. This contradicts the assumption that $\Pi$ is $(f,r;\epsilon)$-resilient.

Note that the above argument stands no matter which group of agents are stragglers (less than $r$), since the existence of stragglers does not change the supposedly \textit{correct} minimum $X_S$ or $X_{\widehat{S}\cup T'}$, the minimum of aggregate of non-faulty cost functions. \qedhere
\end{proof}


With Theorem~\ref{thm:necc}, we show that $(f,r;\epsilon)$-resilience can only be guaranteed with at least $(f,r;\epsilon)$-redundancy in the local cost functions. That is, it is possible to approximate the optimization problem resiliently, and the accuracy of the approximation is related to the redundancy in cost functions. This result motivates us to further explore practical solutions that achieves certain degree of resilience for RDO problems.
